EVOLUTION OF IR-SELECTED GALAXIES IN Z~0.4 CLUSTERS

Wide-field optical and near--IR ($JHK$) imaging is presented for two rich galaxy clusters: Abell~370 at $z=0.374$ and Abell~851 (Cl0939+47) at $z=0.407$. Galaxy catalogs selected from the near--IR images are 90\% complete to approximately 1.5 mag below $K^\ast$ resulting in samples with $\sim$100 probable member galaxies per cluster in the central $\sim$2 Mpc. Comparison with $HST$ WFPC images yields subsamples of $\sim$70 galaxies in each cluster with morphological types. Analysis of the complete samples and the $HST$ subsamples shows that the $z\sim 0.4$ E/S0s are bluer than those in the Bower et al.\ (1992) Coma sample in the optical$-K$ color by $0.13$~mag for Abell~370 and by $0.18$~mag for Abell~851. If real, the bluing of the E/S0 populations at moderate redshift is consistent with that calculated from the Bruzual and Charlot (1993) models of passive elliptical galaxy evolution. In both clusters the intrinsic scatter of the known E/S0s about their optical$-K$ color--mag relation is small ($\sim 0.06$ mag) and not significantly different from that of Coma E/S0s as given by Bower et al.\ (1992), indicating that the galaxies within each cluster formed at the same time at an early epoch.

==> table1.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother
 
\begin{planotable}{lccccrr}
\tablenum{1}
\tablewidth{0pt}
\tablecaption{Comparison of Coma Photometry\tablenotemark{a}}
\tablehead{
\colhead{Galaxy} & \colhead{J(PFA)} & \colhead{J(SED)} & 
\colhead{H(PFA)} & \colhead{H(SED)} & \colhead{K(PFA)} & \colhead{K(SED)} 
}
  
\startdata
~NGC4883 & 12.52 & 12.53 & 11.82 & 11.84 & 11.56 & 11.57 \nl
~NGC4886 & 12.65 & 12.63 & 11.94 & 11.93 & 11.70 & 11.73 \nl
~NGC4889 & 11.03 & 10.97 & 10.28 & 10.26 & 9.99 & 9.98 \nl
~IC4011 & 13.27 & 13.26 & 12.61 & 12.57 & 12.32 & 12.32 \nl
~IC4021 & 12.89 & 12.90 & 12.17 & 12.18 & 11.94 & 11.91 \nl

\tablenotetext{a}{PFA is Persson et al.\ (1979), and
SED is this paper.}

\end{planotable}


==> table2.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

\begin{planotable}{ccrrcccccc}
\tablenum{2}
\tablewidth{0pt}
\tablecaption{Abell 370 Photometry}
\tablehead{
\colhead{SED} & \colhead{BO} & \colhead{~~~x(\arcsec)} &
\colhead{~~~y(\arcsec)} & \colhead{M} & \colhead{Type} & \colhead{~K}  &
\colhead{~H} & \colhead{~J}  & \colhead{7512--K}}

\startdata
%
   18 & \nodata &   91.6 &  19.6 & \nodata & $\ast$ &  10.97
 &  11.03 &  11.55 &   2.10\nl
   19 & \nodata & --47.3 &  --51.5 & \nodata & $\ast$ &  12.57
 &  12.60 &  12.91 &   1.06\nl
   20 & \nodata &   25.4 &  102.0 & \nodata & \nodata &  12.81
 &  13.09 &  13.83 &   2.40\nl
   21 & \nodata &   100.1 &  136.9 & \nodata & $\ast$ &  14.19
 &  14.34 &  14.95 &   1.62\nl
   22 & \nodata & --120.0 &  19.2 & \nodata & $\ast$ &  15.05
 &  15.06 &  15.32 &   0.67\nl
%
   23\tablenotemark{a} &    10 &    0.0 &    0.0 &  SM & E &  15.12
 &  15.73 &  16.65 &   3.08\nl
%
   24 &     6 &   10.1 &  58.4 &  \nodata & E &  15.18
 &  15.56 &  16.30 &   2.41\nl
%
   25 &     9 &    6.5 & --35.5 &  SM & E &  15.20
 &  15.82 &  16.72 &   2.98\nl
%
   26 &  14 & --121.9 &  65.9 &  SM & \nodata &  15.26
 &  15.89 &  16.76 &   2.99\nl
%
   27 & \nodata &   65.2 &  62.6 &  \nodata & \nodata &  15.67
 &  15.86 &  16.49 &   2.28\nl
%
   28 & \nodata & --112.5 &  90.3 &  \nodata & \nodata &  15.68
 &  16.25 &  17.11 &   2.86\nl
%
   29 & 31 &   62.6 &  77.6 &  SM & \nodata &  15.69
 &  16.39 &  17.32 &   3.15\nl
%
   30 & 15 &  --61.6 &  36.2 &  SNM & \nodata &  15.71
 &  16.26 &  17.08 &   2.77\nl
%
   31 &  \nodata & 52.8 & --9.1 &  SM & E &  15.73
 &  16.37 &  17.26 &   3.00\nl
%
   32 &    29 &  --19.9 & --31.9 &  \nodata & L &  15.77
 &  16.41 &  17.34 &   3.01\nl
%
   33 & 22 &   76.3 &  73.7 &  SM & \nodata &  15.78
 &  16.36 &  17.29 &   2.94\nl
%
   34 &    21 &  --57.0 & --15.0 &  SM & L &  15.81
 &  16.39 &  17.28 &   2.95\nl
%
   35 & \nodata &  135.3 &  30.6 &  \nodata & \nodata &  15.82
 &  16.02 &  16.64 &   2.21\nl
%
   36 &    34 &  --27.4 &  24.5 &  SM & L &  15.85
 &  16.48 &  17.36 &   3.05\nl
%
   37 &    26 &   37.2 &  13.4 &  SM & E &  15.86
 &  16.49 &  17.40 &   3.05\nl
%
   38 & \nodata & --112.5 & 110.2 &  \nodata & \nodata &  15.86
 &  16.22 &  16.90 &   2.28\nl
%
   39 &    24 &   --3.6 &  35.2 &  SM & E &  15.88
 &  16.53 &  17.40 &   2.99\nl
%
   40 & 36 &   77.3 & --79.2 &  SM & \nodata &  15.92
 &  16.55 &  17.49 &   3.01\nl
%
   41 & 32 &  120.3 & --51.8 &  SM & \nodata &  15.97
 &  16.60 &  17.54 &   2.98\nl
%
   42 &    58 &   --1.0 &  --5.9 & SNM & L &  15.98
 &  16.60 &  17.49 &   3.20\nl
%
   43 & \nodata &   73.0 &  20.9 &  SNM & $\ast$ &  16.04
 &  16.10 &  16.53 &   1.16\nl
%
   44 &    41 &   44.3 &    0.0 &  SM & L &  16.08
 &  16.72 &  17.64 &   3.06\nl
%
   45 & 20 &    2.6 & --86.7 & SNM & $\ast$ &  16.11
 &  16.35 &  16.91 &   2.50\nl
%
   46 &    43 &   27.1 &  23.1 &  SM & E &  16.11
 &  16.68 &  17.59 &   2.96\nl
%
   47 &    45 &  --43.7 &  21.2 &  SM & B &  16.23
 &  16.73 &  17.80 &   3.00\nl
%
   48 &  \nodata &   21.8 & --47.6 &  SM & E &  16.26
 &  16.87 &  17.75 &   3.03\nl
%
   49 &    61 &  --12.7 &  --1.0 &  SM & B &  16.31
 &  16.87 &  17.80 &   3.02\nl
%
   50 & 47 &  114.1 &  --121.3 &  SM & \nodata &  16.32
 &  16.92 &  17.82 &   3.06\nl

%
   51 & 50 &  112.8 &  --82.5 &  SM & \nodata &  16.35
 &  16.95 &  17.91 &   2.96\nl
%
   52 &    63 &   --1.6 &  --23.5 &  SM & B &  16.36
 &  16.96 &  17.89 &   3.00\nl
%
   53 &  \nodata &    0.3 &  --41.1 &  \nodata & B &  16.36
 &  16.92 &  17.86 &   2.94\nl
%
   54 &    49 &   10.1 &  --43.0 &  \nodata & E &  16.38
 &  16.89 &  17.78 &   2.81\nl
%
   55 &    66 &  --17.3 &  35.9 &  SM & L &  16.40
 &  17.04 &  17.93 &   2.96\nl
%
   56 &    55 &   21.5 &  29.0 &  SM & E &  16.44
 &  17.07 &  17.89 &   2.92\nl
%
   57 &    62 &   51.5 &  --14.7 &  \nodata & E &  16.45
 &  17.05 &  17.92 &   2.90\nl
%
   58 &  \nodata &    3.6 &  --41.1 &  \nodata & E &  16.48
 &  17.13 &  18.02 &   2.99\nl
%
   59 & \nodata & --111.2 & 101.4 &  \nodata & \nodata &  16.48
 &  16.65 &  17.23 &   2.21\nl
%
   60 &    39 &   24.1 &  41.7 &  SM & M &  16.54
 &  17.22 &  18.08 &   2.68 \nl
%
   61 &    60 &  --12.1 & --60.3 &  \nodata & B &  16.54
 &  17.13 &  17.92 &   2.80\nl
%
   62 &    91 &   --0.7 &  --44.7 &  \nodata & E &  16.55
 &  17.24 &  18.18 &   3.06\nl
%
   63 & \nodata &  132.7 &  --70.1 &  \nodata & \nodata &  16.55
 &  17.20 &  18.17 &   2.99\nl
%
   64 & \nodata &  --91.9 & 115.1 &  \nodata & \nodata &  16.55
 &  17.36 &  18.47 &   3.62\nl
%
   65 &    80 &    2.9 &   8.8 &  SM & L &  16.55
 &  17.15 &  18.12 &   3.02\nl

%
   66 &    71 &    1.0 &  --73.3 &  \nodata & A &  16.56
 &  17.13 &  18.11 &   2.87\nl
%
   67 & 96 &   66.8 &  --64.5 &  SM & \nodata &  16.57
 &  17.25 &  18.13 &   3.02\nl
%
   68 & \nodata &  103.3 &  --41.1 &  \nodata & \nodata &  16.58
 &  16.63 &  17.04 &   0.99\nl
%
   69 & \nodata & --136.3 &  49.6 &  \nodata & \nodata &  16.60
 &  16.59 &  16.95 &   0.90\nl
%
   70 & \nodata &   90.0 & 132.4 &  \nodata & \nodata &  16.62
 &  17.23 &  18.14 &   2.82\nl
%
   71 &  \nodata &  --22.8 &  20.9 &  SM & B &  16.63
 &  17.23 &  18.12 &   2.94\nl
%
   72 &    84 &  --16.0 &   2.0 &  \nodata & E &  16.65
 &  17.24 &  18.16 &   2.88\nl
%
   73 & \nodata &  --36.5 &  47.3 &  \nodata & \nodata &  16.66
 &  16.91 &  17.44 &   2.30\nl
%
   74 &    70 &   75.0 &  --13.4 &  SM & L &  16.67
 &  17.29 &  18.14 &   2.83\nl
%
   75 &  \nodata &   --6.5 &  --51.8 &  \nodata & A &  16.69
 &  17.28 &  18.17 &   2.93\nl
%
   76 &   106 &   57.7 &  --43.4 &  SM & E &  16.70
 &  17.32 &  18.28 &   3.01\nl
%
   77 &  75 &   14.0 &  --93.2 &  SM & L &  16.70
 &  17.31 &  18.13 &   2.91\tablebreak
%

   78 &  \nodata &   --4.2 &  --9.5 &  SM & L &  16.71
 &  17.24 &  18.16 &   2.97\nl
%
   79 &  \nodata &    5.5 &  --45.0 &  \nodata & B &  16.72
 &  17.36 &  18.30 &   3.05\nl
%
   80 & \nodata &  --25.4 &  --81.2 &  \nodata & \nodata &  16.74
 &  17.59 &  18.53 &   3.66\nl
%
   81 &   111 &   40.1 &  --2.3 &  \nodata & E &  16.76
 &  17.39 &  18.27 &   3.02\nl
%
   82 & \nodata &  --67.2 &  43.0 &  SNM & \nodata &  16.78
 &  17.41 &  18.15 &   2.70\nl
%
   83 & 79 &   72.4 & --116.7 &  SM & \nodata &  16.78
 &  17.37 &  18.20 &   2.71\nl
%
   84 & 44 &  --10.1 & --109.9 & SNM & \nodata &  16.79
 &  17.35 &  18.21 &   2.79\nl
%
   85 & \nodata &  --84.8 &  60.0 & SNM & $\ast$ &  16.80
 &  16.71 &  16.95 &   0.55\nl
%
   86 &   119 &   26.7 &  --34.2 &  \nodata & L &  16.82
 &  17.41 &  18.42 &   3.18\nl
%
   87 & 99 &  --48.2 &  17.6 &  SNM & \nodata &  16.87
 &  17.42 &  18.39 &   2.96\nl
%
   88 & \nodata &  113.4 & --131.1 &  \nodata & \nodata &  16.89
 &  17.59 &  18.64 &   2.97\nl
%
   89 & \nodata &   73.3 & 113.8 &  \nodata & \nodata &  16.90
 &  17.55 &  18.46 &   2.80\nl
%
   90 & 59 &  119.6 &  --109.9 &  SNM & \nodata &  16.90
 &  17.49 &  18.23 &   2.46\nl
%
   91 & \nodata & --108.6 &  38.8 &  SM & \nodata &  16.91
 &  17.44 &  18.42 &   2.85\nl
%
   92 &   154 &  --17.0 &  --29.0 &  \nodata & E &  16.91
 &  17.44 &  18.20 &   2.97\nl
%
   93 & 130 &  --17.3 &  --66.8 & SNM & B &  16.91
 &  17.57 &  18.34 &   3.06\nl
%
   94 & \nodata &  104.0 &  80.2 &  \nodata & \nodata &  16.93
 &  17.54 &  18.47 &   3.09\nl
%
   95 &   131 &  --29.7 &  34.6 &  SM & L &  16.97
 &  17.71 &  18.66 &   3.01\nl
%
   96 &  \nodata &  --15.6 &  --13.0 &  \nodata & E &  16.99
 &  17.61 &  18.41 &   2.86\nl
%
   97 & 102 &  --69.4 &  --21.5 &  SM & \nodata &  16.99
 &  17.55 &  18.44 &   2.88\nl
%
   98 & \nodata &  --25.4 & 128.4 &  \nodata & \nodata &  17.00
 &  17.62 &  18.40 &   2.67\nl
%
   99 &  \nodata &   27.1 &  --15.3 &  \nodata & E &  17.00
 &  17.69 &  18.59 &   3.04\nl
%
  100 &    95 &   --3.9 &  --68.1 &  \nodata & E &  17.01
 &  17.52 &  18.31 &   2.72\nl
%
  101 &   152 &  --16.3 &  --63.9 &  \nodata & L &  17.02
 &  17.74 &  18.47 &   3.04\nl
%
  102 &   107 &    7.2 &  66.2 &  SM & L &  17.05
 &  17.61 &  18.53 &   2.81\nl
%
  103 & \nodata &  --13.7 & 118.0 &  \nodata & \nodata &  17.06
 &  17.81 &  18.63 &   2.99\nl
%
  104 &   190 &   29.7 & --7.8 &  \nodata & E &  17.07
 &  17.81 &  18.67 &   3.06 \nl
%
  105 & 56 & --121.9 &  7.2 & SNM & \nodata &  17.10
 &  17.46 &  18.24 &   2.32\nl
%
  106 & 108 &  --64.2 &  --76.9 &  SM & \nodata &  17.12
 &  17.72 &  18.62 &   2.78\nl
%
  107 &   136 &    5.9 &  --51.5 &  SM & E &  17.12
 &  17.70 &  18.52 &   2.83\nl
%
  108 &   230 &   --5.2 &  --12.4 &  \nodata & E &  17.12
 &  17.82 &  18.83 &   3.19\nl
%
  109 &   149 &   52.2 &  19.2 &  SM & A &  17.13
 &  17.64 &  18.54 &   2.89\nl
%
  110 & \nodata &    8.5 &  --30.3 &  \nodata & \nodata &  17.13
 &  17.78 &  18.66 &   2.70\nl
%
  111 &   129 &   26.4 &  --44.0 &  \nodata & C &  17.14
 &  17.69 &  18.61 &   2.80\nl
%
  112 & \nodata &  109.9 &  --76.0 &  \nodata & \nodata &  17.16
 &  17.81 &  18.81 &   3.06\nl
%
  113 & \nodata &    2.0 &  92.3 &  \nodata & \nodata &  17.17
 &  17.72 &  18.58 &   2.77\nl
%
  114 &   165 &   30.0 &  --32.6 &  SM & C &  17.17
 &  17.75 &  18.74 &   2.85\nl
%
  115 &   105 &   28.4 &  --20.5 &  \nodata & E &  17.20
 &  17.76 &  18.56 &   2.62\nl
%
  116 & 113 & --120.0 &  --30.6 & SNM & \nodata &  17.20
 &  17.71 &  18.55 &   2.72\nl
%
  117 & 167 &  --27.4 &  --74.7 &  SM & A &  17.22
 &  17.99 &  18.69 &   3.04\nl
%
  118 & \nodata &   77.9 & 103.7 &  \nodata & \nodata &  17.24
 &  17.86 &  18.58 &   2.66\nl
%
  119 & \nodata &   71.7 & 110.2 &  \nodata & \nodata &  17.27
 &  18.03 &  18.86 &   2.90\nl
%
  120 & \nodata &  108.2 & 126.2 &  \nodata & \nodata &  17.28
 &  18.22 &  19.35 &   3.82\nl
%
  121 &   161 &   39.4 &  --25.1 &  \nodata & L &  17.28
 &  17.86 &  18.81 &   2.80\nl
%
  122 &   142 &  --14.0 &  --49.2 &  SM & L &  17.31
 &  17.82 &  18.63 &   2.82\nl
%
  123 &   128 &  --25.1 &  31.9 &  SM & M &  17.32
 &  17.98 &  18.75 &   2.50\nl
%
  124 &  \nodata &   15.0 &  --42.4 &  SNM & D &  17.32
 &  18.04 &  18.90 &   2.93\nl
%
  125 &   153 &   36.5 &  26.7 &  \nodata & E &  17.33
 &  17.79 &  18.89 &   2.96\nl
%
  126 &   133 &   19.2 &  --17.0 &  SM & L &  17.37
 &  18.03 &  19.14 &   2.88\nl
%
  127 & 145 &  --94.5 &  12.4 &  SM & \nodata &  17.37
 &  17.88 &  18.83 &   2.66\nl
%
  128 & \nodata &   73.3 &  67.2 &  \nodata & \nodata &  17.39
 &  18.15 &  19.10 &   3.21\nl
%
  129 &   166 &  --38.5 &  2.9 &  SM & L &  17.40
 &  17.95 &  18.64 &   2.61\nl
%
  130 &   203 &   70.1 &  --21.5 &  \nodata & E &  17.41
 &  18.18 &  18.97 &   3.02\nl

%
  131 & \nodata &  128.1 & 129.1 &  \nodata & \nodata &  17.42
 &  18.02 &  18.81 &   2.46\nl
%
  132 &  \nodata &   --8.5 &  --87.4 &  \nodata & A &  17.42
 &  18.15 &  18.96 &   2.90\nl
%
  133 &   219 &   16.3 &   --4.2 &  \nodata & B &  17.44
 &  18.34 &  19.52 &   3.17\nl
%
  134 &  \nodata &  --18.6 &  --2.0 &  \nodata & E &  17.44
 &  18.01 &  18.78 &   2.84\nl
%
  135 &   232 &   13.4 &  --12.7 &  \nodata & B &  17.52
 &  18.44 &  19.61 &   2.99\tablebreak
%

  136 & \nodata & --132.0 &  --58.0 &  \nodata & \nodata &  17.53
 &  18.08 &  19.04 &   2.73\nl
%
  137 & \nodata &  --92.9 &  52.5 &  \nodata & \nodata &  17.54
 &  18.19 &  19.13 &   3.02\nl
%
  138 & \nodata &  113.8 &  28.4 &  \nodata & \nodata &  17.54
 &  18.15 &  19.10 &   2.66\nl
%
  139 &  \nodata &   79.2 &  16.6 &  \nodata & L &  17.55
 &  18.00 &  18.81 &   2.62\nl
%
  140 & \nodata &  116.1 &  65.5 &  \nodata & \nodata &  17.55
 &  18.17 &  19.13 &   3.45\nl
%
  141 & \nodata &   --1.6 & 136.6 &  \nodata & \nodata &  17.55
 &  18.14 &  19.36 &   2.99\nl
%
  142 &   163 &   --6.5 &  60.3 &  SM & B &  17.57
 &  18.33 &  19.05 &   2.72\nl
%
  143 & \nodata &   79.5 & 109.5 &  \nodata & \nodata &  17.58
 &  18.10 &  18.67 &   2.54\nl
%
  144 &  \nodata &  --63.9 &  28.7 &  \nodata & B &  17.59
 &  18.45 &  19.02 &   2.94\nl
%
  145 &   213 &   42.1 &  4.2 &  \nodata & L &  17.59
 &  18.04 &  18.92 &   2.86\nl
%
  146 & \nodata &  140.2 &  22.5 &  \nodata & \nodata &  17.61
 &  18.25 &  18.91 &   2.67\nl
%
  147 & \nodata &  --20.9 &  35.9 &  \nodata & \nodata &  17.62
 &  17.98 &  18.41 &   2.43\nl
%
  148 & 137 &   73.7 &  --69.8 &  SM & \nodata &  17.62
 &  18.33 &  19.03 &   2.37\nl
%
  149 & \nodata &  --46.0 & 114.4 &  \nodata & \nodata &  17.63
 &  18.09 &  19.09 &   2.69\nl
%
  150 & \nodata &   --8.5 &  7.8 &  \nodata & \nodata &  17.64
 &  18.37 &  19.17 &   3.38\nl
%
  151 &  \nodata &    2.6 &  --9.1 &  \nodata & E &  17.65
 &  18.24 &  18.95 &   2.96\nl
%
  152 & 16 &  --90.6 &  --51.2 & SNM & $\ast$ &  17.65
 &  17.52 &  17.53 &   0.50\nl
%
  153 & \nodata &   82.2 & --142.1 &  \nodata & \nodata &  17.66
 &  18.56 &  19.12 &   3.16\nl
%
  154 &  \nodata &   --2.0 &  --90.0 &  \nodata & A &  17.69
 &  18.38 &  19.24 &   2.89\nl
%
  155 & \nodata &  112.5 &  --93.2 &  \nodata & \nodata &  17.70
 &  18.60 &  19.38 &   2.93\nl
%
  156 & \nodata &  --84.1 &  87.0 &  \nodata & \nodata &  17.71
 &  18.35 &  19.03 &   2.62\nl
%
  157 &   181 &    9.8 &  --59.7 &  \nodata & B &  17.72
 &  18.19 &  19.14 &   2.67\nl
%
  158 & \nodata &  --68.8 &  --35.2 &  \nodata & \nodata &  17.74
 &  18.53 &  19.47 &   2.94\nl
%
  159 &  \nodata &  --34.2 &  --5.5 &  \nodata & L &  17.76
 &  18.25 &  19.05 &   2.41\nl
%
  160 & \nodata & --132.4 &  38.5 &  \nodata & \nodata &  17.80
 &  18.72 &  20.02 &   3.32\nl
%
  161 & \nodata &  --35.5 & --105.3 &  \nodata & \nodata &  17.81
 &  18.25 &  18.94 &   2.32\nl
%
  162 & \nodata &  --15.0 & 111.5 &  \nodata & \nodata &  17.82
 &  18.65 &  19.51 &   2.86\nl
%
  163 &   197 &   13.7 &  78.6 &  \nodata & E &  17.83
 &  18.39 &  19.38 &   2.73\nl
%
  164 & \nodata & --140.5 &  92.3 &  \nodata & \nodata &  17.83
 &  18.37 &  19.43 &   2.86\nl
%
  165 & \nodata &   81.8 &  --86.7 &  \nodata & \nodata &  17.87
 &  18.55 &  19.32 &   2.93\nl
%
  166 & \nodata &  126.2 & --136.3 &  \nodata & \nodata &  17.87
 &  18.48 &  20.10 &   3.22\nl
%
  167 & \nodata &  107.3 &  --83.1 &  \nodata & \nodata &  17.89
 &  18.66 &  19.05 &   2.44\nl
%
  168 & \nodata &   60.6 & --142.1 &  \nodata & \nodata &  17.89
 &  19.31 &  19.72 &   3.20\nl
%
  169 & \nodata &  --40.1 & --114.4 &  \nodata & \nodata &  17.90
 &  18.22 &  19.16 &   2.21\nl
%
  170 &   236 &   70.7 &  8.2 &  \nodata & B &  17.91
 &  18.58 &  19.61 &   2.90\nl
%
  171 & \nodata &   75.0 & 104.6 &  \nodata & \nodata &  17.92
 &  19.19 &  19.26 &   2.44\nl
%
  172 &   257 &   47.3 &  28.0 &  \nodata & B &  17.92
 &  18.45 &  19.66 &   2.91\nl
%
  173 &   226 &   36.2 &  --26.7 &  \nodata & L &  17.93
 &  18.55 &  19.07 &   2.41\nl
%
  174 & \nodata &  --71.7 & --134.3 &  \nodata & \nodata &  17.94
 &  18.77 &  19.96 &   3.32\nl
%
  175 & \nodata &  140.5 &  --88.3 &  \nodata & \nodata &  17.94
 &  18.64 &  19.59 &   2.92\nl
%
  176 & \nodata & --105.6 & --122.2 &  \nodata & \nodata &  17.95
 &  18.87 &  20.33 &   4.01\nl
%
  177 &   244 &   55.1 &  --60.3 &  \nodata & L &  17.97
 &  18.70 &  19.57 &   2.92\nl
%
  178 &   311 &   42.4 &  --22.2 &  SM & E &  17.98
 &  18.57 &  19.26 &   2.96\nl
%
  179 & \nodata &   55.7 &  57.7 &  \nodata & \nodata &  17.98
 &  18.81 &  20.15 &   4.32\nl
\tablenotetext{a}{J2000: 02\hr 39\min 52\spt50, --01\deg 34\mins 20\arcsec}
\end{planotable}


==> table3.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother

\begin{planotable}{ccrrcccccc}
\tablenum{3}
\tablewidth{0pt}
\tablecaption{Abell 851}
\tablehead{
\colhead{SED} & \colhead{DG} & \colhead{~~~x(\arcsec)} &
\colhead{~~~y(\arcsec)} & \colhead{M} & \colhead{Type} & \colhead{~K}  &
\colhead{~H} & \colhead{~J}  & \colhead{7843--K}}

\startdata

%
   1 & \nodata &  --110.2 &  --95.5 & \nodata & $\ast$  &  13.43
 &  13.51 &  13.83 &   0.88\nl
   2 & \nodata &    89.7 &  111.2 & \nodata & $\ast$  &  14.12
 &  14.16 &  14.53 &   0.77\nl
   3 & \nodata &  109.9 & --102.7 & \nodata & \nodata  &  14.21
 &  14.63 &  15.40 &   2.31\nl
   4 & \nodata &   64.5 & --69.8 & \nodata & $\ast$  &  14.21
 &  14.25 &  14.58 &   0.75\nl
   5 & \nodata &  131.7 &  14.3 & \nodata & \nodata  &  14.89
 &  15.30 &  16.05 &   2.25\nl
   6 & \nodata &  --94.5 & 139.2 & \nodata & \nodata  &  15.53
 &  16.19 &  17.02 &   2.72\nl
%
   7\tablenotemark{a} &   311 &    0.0 &    0.0 &  SM & E &  15.55
 &  16.21 &  17.05 &   2.79\nl
%
   8 &   439 &  --16.3 &  47.3 &  SM & M &  15.68
 &  16.26 &  17.14 &   2.58\nl
%
   9 &   367 &  --12.4 &  21.2 &  SM & E &  15.86
 &  16.55 &  17.40 &   2.85\nl
%
  10 &   366 &    4.9 &  21.5 &  SM & E &  15.86
 &  16.46 &  17.35 &   2.78\nl
%
  11 &   296 &  --22.2 &  --8.5 &  \nodata & B &  15.86
 &  16.63 &  17.67 &   3.41\nl
%
  12 &   396 &  104.0 &  34.9 & SNM & L &  15.88
 &  16.46 &  17.30 &   2.61\nl
%
  13 &   236 &   65.9 & --31.0 & \nodata & $\ast$  &  15.96
 &  16.19 &  16.78 &   2.08\nl
%
  14 & \nodata &  --69.8 &  22.8 & \nodata & \nodata  &  15.99
 &  16.42 &  17.09 &   2.13\nl
%
  15 &   460 &   75.0 &  59.7 &  SM & E &  15.99
 &  16.58 &  17.49 &   2.81\nl
%
  16 & \nodata &  --28.4 &  --13.0 & \nodata & \nodata  &  16.00
 &  16.59 &  17.44 &   2.75\nl
%
  17 & \nodata &   58.4 & 139.9 & \nodata & \nodata  &  16.01
 &  16.62 &  17.59 &   2.88\nl
%
  18 & \nodata &  --88.3 & 135.6 & \nodata & \nodata  &  16.10
 &  16.78 &  17.65 &   2.75\nl
%
  19 &     360 &   --7.8 &  18.6 &  SM &  A  &  16.14
 &  16.80 &  17.61 &   2.70\nl
%
  20 & \nodata &  135.3 & --7.2 & \nodata & \nodata  &  16.18
 &  16.74 &  17.59 &   2.60\nl
%
  21 & \nodata &   89.3 & --102.0 & \nodata & \nodata  &  16.18
 &  16.36 &  16.97 &   2.06\nl
%
  22 &   270 &   37.2 &  --17.3 & SNM & B &  16.31
 &  16.88 &  17.60 &   2.47\nl
%
  23 & \nodata & --112.1 & 158.8 & \nodata & \nodata  &  16.32
 &  17.05 &  17.72 &   9.85\nl
%
  24 & \nodata &   21.5 &  87.7 & \nodata & \nodata  &  16.32
 &  16.88 &  17.88 &   2.65\nl
%
  25 & \nodata &   45.0 & 129.7 & \nodata & \nodata  &  16.34
 &  16.99 &  17.83 &   2.63\nl
%
  26 &   398 &   88.0 &  34.9 & SNM & E &  16.35
 &  17.00 &  17.91 &   2.88\nl
%
  27 & \nodata &  --11.7 & --109.2 & \nodata & \nodata  &  16.39
 &  17.01 &  17.82 &   2.65\nl
%
  28 & \nodata &  135.6 &  --17.6 & \nodata & \nodata  &  16.42
 &  16.96 &  17.86 &   2.68\nl
%
  29 & \nodata & --105.3 &  16.6 & \nodata & \nodata  &  16.44
 &  17.10 &  17.92 &   2.65\nl
%
  30 &   393 &   52.2 &  33.3 &  SM & E &  16.45
 &  17.06 &  17.95 &   2.77\nl
%
  31 & \nodata &    5.2 & 127.8 & \nodata & \nodata  &  16.46
 &  16.98 &  17.93 &   2.51\nl
%
  32 & \nodata & --126.5 & 109.2 & \nodata & \nodata  &  16.47
 &  17.12 &  18.14 &   2.98\nl
%
  33 &   241 &    4.2 & --28.4 &  \nodata & L &  16.47
 &  17.10 &  18.01 &   2.70\nl
%
  34 & \nodata &    4.6 &  95.8 & \nodata & \nodata  &  16.48
 &  16.56 &  17.19 &   1.51\nl
%
  35 &   188 &  --19.9 &  --52.2 &  \nodata & A &  16.53
 &  17.06 &  17.97 &   2.56\nl
%
  36 & \nodata &   65.2 & 124.9 & \nodata & \nodata  &  16.57
 &  17.26 &  18.32 &   3.15\nl
%
  37 & \nodata &   43.4 &  --21.2 & \nodata & $\ast$  &  16.60
 &  16.76 &  17.06 &   0.87\nl
%
  38 &   436 &   38.1 &  47.6 &  \nodata & L &  16.64
 &  17.32 &  18.24 &   2.72\nl
%
  39 & \nodata &   38.8 &  98.5 & \nodata & \nodata  &  16.66
 &  17.32 &  18.10 &   2.45\nl
%
  40 &   427 &  113.1 &  45.3 &  SM & E &  16.66
 &  17.21 &  18.19 &   2.68\nl
%
  41 &   157 &   --4.9 & --66.5 &  SM & A &  16.66
 &  17.31 &  18.17 &   2.80\nl
%
  42 & \nodata & --108.2 & 153.9 & \nodata & \nodata  &  16.71
 &  17.28 &  18.12 &   2.53\nl
%
  43 & \nodata &  --55.4 & --47.6 & \nodata & \nodata  &  16.71
 &  16.83 &  17.43 &   1.54\nl
%
  44 &   397 &   42.7 &  33.6 &  \nodata & L &  16.76
 &  17.40 &  18.31 &   2.90\nl
%
  45 &   206 &    6.2 &  --44.7 &  \nodata & E &  16.76
 &  17.55 &  18.43 &   2.84\nl
%
  46 & \nodata &  --17.9 & 121.6 & \nodata & \nodata  &  16.78
 &  16.80 &  17.40 &   1.36\nl
%
  47 &   422 &  --17.9 &  40.4 &  SM & L &  16.80
 &  17.42 &  18.18 &   2.57\nl
%
  48 &   226 &   17.3 &  --35.9 &  \nodata & L &  16.81
 &  17.44 &  18.37 &   2.75\nl
%
  49 &   234 &   73.0 &  --31.3 & SNM & B &  16.82
 &  17.48 &  18.26 &   2.69\nl
%
  50 &   310 &   91.3 &  1.6 &  SM & E &  16.82
 &  17.44 &  18.33 &   2.73\nl
%
  51 &   282 &  --20.9 &  --13.4 &  \nodata & B &  16.82
 &  17.46 &  18.37 &   2.92\nl
%
  52 &   519 &   --6.5 &  76.0 &  SM & \nodata  &  16.83
 &  17.42 &  18.35 &   2.83\nl
%
  53 & \nodata &  --51.8 & 100.7 & \nodata & \nodata  &  16.84
 &  17.39 &  18.24 &   2.70\nl
%
  54 &   349 &   78.2 &  16.6 & SNM & L &  16.86
 &  17.51 &  18.32 &   2.58\nl
%
  55 &   279 &  --14.0 & --14.3 &  SM & L &  16.94
 &  17.58 &  18.58 &   2.76\nl
%
  56 & \nodata &   54.4 & --120.9 & SNM & \nodata  &  17.00
 &  17.93 &  19.07 &   3.53\nl
%
  57 & \nodata & --123.2 &  5.9 & \nodata & \nodata  &  17.02
 &  17.42 &  18.32 &   2.48\nl
%
  58 &   303 &   99.8 & --1.6 &  \nodata & L &  17.04
 &  17.59 &  18.52 &   2.62\nl
%
  59 & \nodata &  --62.3 & 137.9 & \nodata & \nodata  &  17.06
 &  17.78 &  18.61 &   2.76\nl
%
  60 & \nodata &   31.6 &  94.5 & \nodata & \nodata  &  17.08
 &  17.68 &  18.49 &   2.68\nl
%
  61 & \nodata &  --82.8 & 125.8 & \nodata & \nodata  &  17.09
 &  17.74 &  18.65 &   2.71\nl
%
  62 & \nodata &  --17.9 &  --89.0 & \nodata & \nodata  &  17.09
 &  17.85 &  18.89 &   3.18\tablebreak
%

  63 & \nodata &    1.0 &  62.6 & \nodata & \nodata  &  17.11
 &  17.18 &  17.73 &   1.66\nl
%
  64 & \nodata &  --29.3 &  20.9 & \nodata & \nodata  &  17.12
 &  17.77 &  18.52 &   2.52\nl
%
  65 &   320 &   26.1 &  3.3 &  SM &  M  &  17.14
 &  17.73 &  18.65 &   2.52\nl
%
  66 & \nodata &   57.4 & 150.3 & \nodata & \nodata  &  17.15
 &  17.95 &  18.67 &   2.67\nl
%
  67 & \nodata &   51.2 & --119.0 & \nodata & \nodata  &  17.15
 &  18.17 &  19.00 &   3.26\nl
%
  68 & \nodata &  --53.5 & 129.7 & \nodata & \nodata  &  17.16
 &  17.70 &  18.56 &   2.39\nl
%
  69 & \nodata & --108.6 &  67.5 & \nodata & \nodata  &  17.19
 &  17.70 &  18.37 &   2.37\nl
%
  70 & \nodata & --129.7 & 105.3 & \nodata & \nodata  &  17.20
 &  18.10 &  18.87 &   3.13\nl
%
  71 & \nodata &  156.5 & 140.5 & \nodata & \nodata  &  17.20
 &  17.93 &  18.90 &   9.37\nl
%
  72 & \nodata &   23.8 & 143.8 & \nodata & \nodata  &  17.21
 &  17.90 &  18.50 &   2.28\nl
%
  73 &   381 &   60.0 &  27.4 &  \nodata & L &  17.22
 &  17.95 &  18.84 &   2.81\nl
%
  74 & \nodata &   --4.2 & 115.4 & \nodata & \nodata  &  17.25
 &  17.80 &  18.78 &   2.49\nl
%
  75 &   135 &   72.0 &  --78.9 &  SM & B &  17.26
 &  17.74 &  18.64 &   2.51\nl
%
  76 & 432 &   --0.3 &  45.3 &  SM &  L  &  17.26
 &  18.14 &  18.85 &   2.84\nl
%
  77 & \nodata &  --37.2 &  --30.6 & \nodata & \nodata  &  17.26
 &  17.82 &  18.66 &   2.65\nl
%
  78 &   243 &   --6.5 &  --28.0 &  \nodata & D &  17.27
 &  17.79 &  18.63 &   2.39\nl
%
  79 & \nodata &  --51.8 &  48.2 & \nodata & \nodata  &  17.27
 &  17.66 &  18.71 &   2.73\nl
%
  80 & \nodata &   64.2 &  67.5 & \nodata & \nodata  &  17.30
 &  17.72 &  18.49 &   2.56\nl
%
  81 & 191 &   54.4 &  --50.5 &  SM & L  &  17.30
 &  18.03 &  18.84 &   2.64\nl
%
  82 & \nodata & --127.5 &  --33.6 & \nodata & \nodata  &  17.31
 &  17.99 &  18.86 &   2.76\nl
%
  83 & 511 &   23.8 &  73.7 &  SM & \nodata  &  17.33
 &  18.14 &  18.81 &   2.42\nl
%
  84 & \nodata &  --33.3 &  4.6 & \nodata & \nodata  &  17.33
 &  17.90 &  18.80 &   2.65\nl
%
  85 & \nodata &   98.5 & 116.7 & \nodata & \nodata  &  17.34
 &  17.90 &  18.76 &   2.42\nl
%
  86 &   244 &    8.8 &  --27.7 & SNM & A &  17.34
 &  17.97 &  18.89 &   2.81\nl
%
  87 &   451 &    1.3 &  52.8 &  SM & M &  17.35
 &  18.07 &  18.93 &   2.61\nl
%
  88 & \nodata &  --69.4 & 112.5 & \nodata & \nodata  &  17.35
 &  17.88 &  18.60 &   1.89\nl
%
  89 & \nodata &   58.7 & 125.8 & \nodata & \nodata  &  17.39
 &  18.11 &  18.89 &   2.72\nl
%
  90 & \nodata &  --86.4 & 119.3 & \nodata & \nodata  &  17.39
 &  17.67 &  18.16 &   2.24\nl
%
  91 &   246 &  101.1 &  --24.5 &  \nodata & L &  17.39
 &  17.94 &  18.94 &   2.92\nl
%
  92 &   390 &  --23.5 &  31.0 &  SM & A &  17.41
 &  17.95 &  18.74 &   2.45\nl
%
  93 & 80 &   55.4 & --116.7 &  SM & \nodata  &  17.42
 &  18.17 &  18.93 &   2.66\nl
%
  94 & \nodata &   81.8 & --124.5 & \nodata & \nodata  &  17.43
 &  18.21 &  19.27 &   6.58\nl
%
  95 &   321 &   --9.5 &  3.9 &  SM & L &  17.44
 &  18.00 &  18.72 &   2.56\nl
%
  96 & \nodata &   16.3 & 122.2 & \nodata & \nodata  &  17.44
 &  18.10 &  19.12 &   2.76\nl
%
  97 & \nodata &  --47.6 &  45.3 & \nodata & \nodata  &  17.45
 &  18.03 &  19.03 &   2.85\nl
%
  98 &   348 &  106.6 &  16.3 &  \nodata & C &  17.47
 &  18.36 &  19.41 &   2.49\nl
%
  99 & 186 &  119.3 &  --47.6 & \nodata & B  &  17.47
 &  18.60 &  19.33 &   3.59\nl
%
 100 & \nodata &  --55.1 & --106.0 & \nodata & \nodata  &  17.50
 &  17.93 &  18.41 &   2.74\nl
%
 101 & \nodata &  125.2 &  77.3 & \nodata & \nodata  &  17.51
 &  18.20 &  18.90 &   2.75\nl
%
 102 &   471 &    6.8 &  60.3 &  SM & C &  17.52
 &  18.29 &  19.05 &   2.41\nl
%
 103 & \nodata &  122.2 &  67.8 & \nodata & \nodata  &  17.53
 &  18.16 &  18.95 &   2.47\nl
%
 104 &   408 &    2.9 &  35.9 &  \nodata & L &  17.56
 &  18.85 &  19.52 &   3.28\nl
%
 105 & \nodata & --100.7 & 131.4 & \nodata & \nodata  &  17.57
 &  18.20 &  19.21 &   2.76\nl
%
 106 & \nodata &  122.2 &  90.6 & \nodata & \nodata  &  17.58
 &  18.12 &  18.89 &   2.61\nl
%
 107 & \nodata &  --53.5 &  --25.1 & \nodata & \nodata  &  17.58
 &  18.12 &  19.21 &   3.05\nl
%
 108 & \nodata &   49.9 & 132.4 & \nodata & \nodata  &  17.58
 &  18.07 &  19.00 &   2.70\nl
%
 109 & \nodata &  --47.6 &  18.3 & \nodata & \nodata  &  17.60
 &  18.10 &  19.01 &   2.61\nl
%
 110 &   380 &   92.3 &  28.4 &  \nodata & A &  17.60
 &  18.28 &  19.19 &   2.69\nl
%
 111 & \nodata &  --62.9 & 118.0 & \nodata & \nodata  &  17.61
 &  18.08 &  18.80 &   2.20\nl
%
 112 &   458 &    4.2 &  55.4 &  \nodata & E &  17.62
 &  18.32 &  18.85 &   2.60\nl
%
 113 &   410 &   --6.8 &  36.5 &  \nodata & L &  17.62
 &  18.27 &  19.06 &   2.68\nl
%
 114 &   338 &  --21.8 &  8.8 &  \nodata & A &  17.62
 &  18.42 &  19.06 &   2.83\nl
%
 115 &   225 &  101.4 & --33.9 &  SM & C &  17.64
 &  18.02 &  19.33 &   2.95\nl
%
 116 &   169 &   12.7 & --60.6 &  \nodata & L &  17.66
 &  18.59 &  19.16 &   2.64\nl
%
 117 & \nodata &   13.4 & 129.7 & \nodata & \nodata  &  17.66
 &  18.19 &  19.02 &   2.09\nl
%
 118 & \nodata & --133.0 &  34.9 & \nodata & \nodata  &  17.67
 &  18.07 &  19.13 &   2.83\nl
%
 119 & \nodata &   24.5 & --128.4 & \nodata & \nodata  &  17.67
 &  18.31 &  19.14 &   7.82\nl
%
 120 &   150 &   74.7 & --70.1 &  SM & A &  17.68
 &  18.18 &  18.94 &   2.53\nl
%
 121 & \nodata & --109.5 &  86.4 & \nodata & \nodata  &  17.69
 &  18.18 &  18.93 &   2.26\nl
%
 122 & \nodata &  --21.2 & 146.4 & \nodata & \nodata  &  17.70
 &  18.45 &  19.22 &   2.73\nl
%
 123 & \nodata &  104.0 & 112.8 & \nodata & \nodata  &  17.72
 &  18.46 &  19.26 &   3.93\tablebreak
%

 124 & \nodata &  --88.7 & --35.9 & \nodata & \nodata  &  17.75
 &  17.85 &  18.34 &   1.86\nl
%
 125 & \nodata &   36.5 & --127.1 & \nodata & \nodata  &  17.76
 &  18.55 &  19.39 &   7.45\nl
%
 126 & \nodata &  --92.6 &  --65.5 & \nodata & \nodata  &  17.78
 &  18.84 &  19.90 &   3.28\nl
%
 127 & \nodata &  132.0 &  --41.7 & \nodata & \nodata  &  17.78
 &  18.51 &  19.51 &   2.79\nl
%
 128 & \nodata &   83.1 &  --85.4 & \nodata & \nodata  &  17.79
 &  18.77 &  19.61 &   2.99\nl
%
 129 &   419 &   46.6 &  41.1 &  \nodata & L &  17.79
 &  18.56 &  19.32 &   2.58\nl
%
 130 &   403 &   59.0 &  35.9 & SNM & C &  17.80
 &  18.65 &  19.20 &   2.47\nl
%
 131 & \nodata &   91.9 &  --90.6 & \nodata & \nodata  &  17.80
 &  18.46 &  19.44 &   2.77\nl
%
 132 &   457 &   97.5 &  57.7 &  \nodata & E &  17.80
 &  18.63 &  19.85 &   2.85\nl
%
 133 &   420 &   38.8 &  41.1 & SNM & B &  17.80
 &  18.62 &  19.33 &   2.54\nl
%
 134 & \nodata &  --63.9 & --35.9 & \nodata & \nodata  &  17.81
 &  17.86 &  18.66 &   1.75\nl
%
 135 & \nodata &  --70.7 &  97.1 & \nodata & \nodata  &  17.82
 &  18.49 &  19.43 &   2.94\nl
%
 136 &   322 &   31.3 &  5.9 &  \nodata & C &  17.83
 &  18.70 &  19.55 &   2.90\nl
%
 137 &   441 &   70.4 & 50.2 &  SM & A &  17.84
 &  18.32 &  18.95 &   2.36\nl
%
 138 & 153 &    3.9 &  --68.5 & \nodata & \nodata  &  17.88
 &  18.41 &  19.23 &   2.38\nl
%
 139 &   176 &  --19.2 &  --59.0 &  \nodata & B &  17.90
 &  18.34 &  19.16 &   2.75\nl
%
 140 & \nodata &   94.9 & 102.4 & \nodata & \nodata  &  17.90
 &  18.28 &  19.32 &   2.10\nl
%
 141 & \nodata &   56.7 & --94.9 & \nodata & \nodata  &  17.91
 &  18.76 &  19.73 &   2.84\nl
%
 142 & \nodata &  144.4 & 136.3 & \nodata & \nodata  &  17.92
 &  18.48 &  19.42 &   2.54\nl
%
 143 & \nodata &  --86.7 & --107.6 & \nodata & \nodata  &  17.93
 &  19.21 &  20.12 &   4.95\nl
%
 144 & \nodata &  --18.6 &  89.3 & \nodata & \nodata  &  17.93
 &  18.64 &  19.41 &   2.68\nl
%
 145 &   143 &   93.6 & --73.7 &  \nodata & M &  17.94
 &  18.01 &  18.62 &   1.98\nl
%
 146 &   375 &   --3.3 &  23.8 &  \nodata & L &  17.94
 &  18.50 &  19.33 &   2.67\nl
%
 147 &   409 &   28.7 &  37.2 &  \nodata & C &  17.94
 &  18.74 &  19.63 &   2.81\nl
%
 148 & \nodata &  102.4 & --107.6 & \nodata & \nodata  &  17.95
 &  18.58 &  19.53 &   2.69\nl
%
 149 &   356 &   37.8 &  17.6 &  \nodata & L &  17.97
 &  18.52 &  19.69 &   2.75\nl
%
 150 & \nodata &   28.4 &  --11.1 & \nodata & \nodata  &  17.97
 &  18.66 &  19.42 &   2.76\nl
%
 151 &   314 &   13.4 &  1.3 &  \nodata & L &  17.98
 &  18.53 &  19.49 &   2.53\nl
%
 152 &   299 &   22.2 & --5.2 &  \nodata & L &  17.98
 &  18.60 &  19.54 &   2.79\nl
%
 153 & \nodata &  --59.0 & --57.0 & \nodata & \nodata  &  17.99
 &  18.27 &  19.35 &   2.60\nl
%
 154 & \nodata &   65.5 & 151.6 & \nodata & \nodata  &  17.99
 &  19.00 &  19.67 &   3.36\nl
\tablenotetext{a}{J2000: 09\hr 42\min 56\spt89, 46\deg 58\mins 44\arcsec}
\end{planotable}


==> table4.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother
 
\begin{planotable}{lll}
\tablenum{4}
\tablewidth{0pt}
\tablecaption{Systematic Errors}
\tablehead{
\colhead{Type} & \colhead{Amount} & \colhead{Affects} } 
  
\startdata
Optical image blur\tablenotemark{a} & 0.01 & our optical mag \nl
Color gradient correction\tablenotemark{b} & 0.02 & Coma $V-H$ \nl
$k$-correction\tablenotemark{c} & 0.01 & Coma $V-H$ \nl
Bower zeropoint uncertainty\tablenotemark{d} & 0.034 & Coma $V-H$ \nl
SED zeropoint uncertainty\tablenotemark{e} & 0.035 &  our optical-$K$ \nl
Reddening correction\tablenotemark{f} & 0.02 & our optical-$K$ \nl
\tablenotetext{a}{Determined using simulated galaxies}
\tablenotetext{b}{Assumes gradients are constant with radius and constant
with luminosity}
\tablenotetext{c}{Determined using BC model elliptical; very similar value
for model disk galaxies}
\tablenotetext{d}{As given by Bower et al.\ (1992) }
\tablenotetext{e}{Using estimates from Burstein \& Heiles (1982)}
\end{planotable}


==> table5.tex <==
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi
\makeatother
 
\begin{planotable}{ccc}
\tablenum{5}
\tablewidth{0pt}
\tablecaption{Median Optical-$K$ Color Residuals from Coma 
as a Function of Morphology for IR/HST Samples}
\tablehead{
\colhead{Type} & \colhead{Abell 370} & \colhead{Abell 851}
}
  
\startdata

E/SO & $-0.13\pm 0.15$ & $-0.18\pm 0.15$ \nl
Sa/Sb  & $-0.11\pm 0.11$ & $-0.26\pm 0.16$ \nl
Sc/Sd & $-0.19\pm 0.07$ & $-0.38\pm 0.25$ \nl

\end{planotable}

